Correlate-and-Excite: Real-Time Stereo Matching via Guided Cost Volume Excitation

Volumetric deep learning approach towards stereo matching aggregates a cost volume computed from input left and right images using 3D convolutions. Recent works showed that utilization of extracted image features and a spatially varying cost volume aggregation complements 3D convolutions. However, existing methods with spatially varying operations are complex, cost considerable computation time, and cause memory consumption to increase. In this work, we construct Guided Cost volume Excitation (GCE) and show that simple channel excitation of cost volume guided by image can improve performance considerably. Moreover, we propose a novel method of using top-k selection prior to soft-argmin disparity regression for computing the final disparity estimate. Combining our novel contributions, we present an end-to-end network that we call Correlate-and-Excite (CoEx). Extensive experiments of our model on the SceneFlow, KITTI 2012, and KITTI 2015 datasets demonstrate the effectiveness and efficiency of our model and show that our model outperforms other speed-based algorithms while also being competitive to other state-of-the-art algorithms. Codes will be made available at https://github.com/antabangun/coex.

==> Tables/Ablation.channel.tex <==
\begin{table}[h]
    \begin{center}
        \begin{tabular}{c|c|c}
            \Xhline{3\arrayrulewidth}
            & Multiplication & Addition\\
            \hline
            Sceneflow EPE & 0.79 & 0.82 \\
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        % \end{adjustbox}
    \caption{Cost volume channel update.}
    \label{table:channel}
    \end{center}
\end{table}

==> Tables/Ablation.cost.tex <==
% \begin{table}[t]
% % \scriptsize
%     \begin{center}
%         \begin{adjustbox}{width=0.48\textwidth}
%         % \renewcommand{\arraystretch}{1.5}
%         % \setlength{\tabcolsep}{4pt}
%         \begin{tabular}{cccccc}
%             \Xhline{3\arrayrulewidth}
%             \multicolumn{5}{c}{SceneFlow EPE} &  \\ 
%             \cmidrule(l{2pt}r{2pt}){2-5} \cmidrule(l{2pt}r{2pt}){6}
%             & \multicolumn{4}{c}{disparity regression $k$} & Time \\
%             & 48 & 6 & 3 & 2 & $ms$ \\
%             \Xhline{2\arrayrulewidth}
%             % \hline
%             baseline & 1.020 & 0.933 & 0.901 & 0.895 & 26  \\
%             Neighbor & 0.895 & 0.838 & 0.822 & 0.819 & 60 \\
%             % \rowcolor{CuGray}
%             GCE & 0.863 & 0.804 & 0.800 & 0.771 & 26 \\
%             \Xhline{3\arrayrulewidth}
%         \end{tabular}
%         \end{adjustbox}
%     \caption{Ablation study of GCE and top-$k$ regression strategy.}
%     \vspace{-7mm}
%     \label{table:topk}
%     \end{center}
% \end{table}


\begin{table}[t]
% \scriptsize
    \begin{center}
        \begin{adjustbox}{width=0.48\textwidth}
        % \renewcommand{\arraystretch}{1.5}
        % \setlength{\tabcolsep}{4pt}
        \begin{tabular}{c|c|c|c|c|c}
            \Xhline{3\arrayrulewidth}
            \multicolumn{5}{c|}{SceneFlow EPE} &  \\ 
            \Xhline{3\arrayrulewidth}
            & \multicolumn{4}{c|}{disparity regression $k$} & Time \\
            & 48 & 6 & 3 & 2 & $ms$ \\
            \Xhline{2\arrayrulewidth}
            % \hline
            baseline & 1.020 & 0.933 & 0.901 & 0.895 & 26  \\
            Neighbor & 0.895 & 0.838 & 0.822 & 0.819 & 60 \\
            % \rowcolor{CuGray}
            GCE & 0.863 & 0.804 & 0.800 & 0.771 & 26 \\
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Ablation study of GCE and top-$k$ regression strategy.}
    \vspace{-7mm}
    \label{table:topk}
    \end{center}
\end{table}


% \begin{table}[t]
% % \scriptsize
%     \begin{center}
%         \begin{adjustbox}{width=0.5\textwidth}
%         % \renewcommand{\arraystretch}{1.5}
%         % \setlength{\tabcolsep}{8pt}
%         \begin{tabular}{c|c|c|c|c|c|c}
%             \Xhline{3\arrayrulewidth}
%             & & & \multicolumn{4}{c}{SceneFlow EPE}  \\ 
%             \cline{4-7}
%             & \multirow{3}{*}{GCE} & \multirow{3}{*}{GSA} & \multicolumn{4}{c}{\cellcolor{CuGray}Top-$k$ regression}  \\
%             \cline{4-7}
%             & & & \multicolumn{4}{c}{$k$}  \\
%             \cline{4-7}
%             & & & 48 & 6 & 3 & 2  \\
%             \Xhline{2\arrayrulewidth}
%             % \hline
%             baseline & & & 1.00 & 0.899 & 0.875 & 0.838  \\
%             \Xhline{2\arrayrulewidth}
%             \cellcolor{CuGray}Self- & \checkmark &  & 0.821 & 0.782 & 0.742 & 0.739  \\
%             \cellcolor{CuGray}updates &  & \checkmark & 0.862 & 0.801 & 0.790 & 0.759 \\
%             \cellcolor{CuGray} & \checkmark & \checkmark & 0.819 & 0.766 & 0.748 & 0.721 \\
%             \Xhline{3\arrayrulewidth}
%         \end{tabular}
%         \end{adjustbox}
%     \caption{Ablation study of top-$k$ regression strategy.}
%     \label{table:topk}
%     \end{center}
% \end{table}



==> Tables/Ablation.gsa.tex <==
\begin{table}[t]
% \scriptsize
    \begin{center}
        \begin{adjustbox}{width=0.5\textwidth}
        % \renewcommand{\arraystretch}{1.5}
        % \setlength{\tabcolsep}{14pt}
        \begin{tabular}{c|c|c|c|c|c}
            \Xhline{3\arrayrulewidth}
            & \multicolumn{3}{c|}{GSA} & \multirow{3}{*}{GCE} & \\
            \cline{2-4}
                    & \multicolumn{3}{c|}{Guide} & & SceneFlow \\
                    \cline{2-4}
                    & $C^{(s)}$ & $C^{(s')}$ & $I^{(s')}$ & & EPE \\
            \Xhline{2\arrayrulewidth}
            baseline & & & & & 1.00\\
            \Xhline{1\arrayrulewidth}
            \multirow{4}{*}{GSA} & \checkmark & \checkmark & & & 0.954 \\
            %  & \checkmark & \checkmark & & & & 0.954 \\
             & & & \checkmark & & 0.860 \\ %%
            %  & \checkmark & & \checkmark & & & 0.872 \\ 
             & \checkmark & \checkmark & \checkmark & & 0.869 \\ 
            %  & \checkmark & & \checkmark & \checkmark & &  \\
            %  & \checkmark & \checkmark & \checkmark & \checkmark & & 0.862 \\
            \Xhline{1\arrayrulewidth}
            \multirow{3}{*}{Combined} & & & & \checkmark & 0.821 \\
             & & & \checkmark & \checkmark & 0.814 \\ %%
             & \checkmark & \checkmark & \checkmark & \checkmark & 0.821 \\ %%
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Ablation study of GSA using different choice as guidance for weight computation.}
    \label{table:gsa}
    \end{center}
\end{table}

==> Tables/Ablation.neighbor.tex <==
\begin{table}[t]
% \scriptsize
    \begin{center}
        \begin{adjustbox}{width=0.5\textwidth}
        % \renewcommand{\arraystretch}{1.5}
        % \setlength{\tabcolsep}{8pt}
        \begin{tabular}{c|c|c|c|c}
            \Xhline{3\arrayrulewidth}
                    & Neighbor  & \multirow{2}{*}{GCE} & SceneFlow & Runtime \\
                    & agg.   &         & EPE & (ms) \\
            \Xhline{2\arrayrulewidth}
            baseline & & & 1.00 & 31 \\
            \Xhline{2\arrayrulewidth}
            \multirow{2}{*}{$s=1/4$} & \checkmark &  & 0.943 & 34 \\
             &  & \checkmark & 0.935 & 31 \\
            \Xhline{2\arrayrulewidth}
            \multirow{2}{*}{$s=1/16$} & \checkmark &  & 0.879 & 67\\
             &  & \checkmark & 0.861 & 32 \\
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Ablation study of GCE and comparison with image guided neighborhood aggregation.}
    \label{table:neighbor}
    \end{center}
\end{table}

==> Tables/Comparison.tex <==
\begin{table*}[ht]
    \begin{center}
        \begin{adjustbox}{width=0.7\textwidth}
        \setlength{\tabcolsep}{5pt}
        \begin{tabular}{c|c|c|c|c|c}
            \Xhline{4\arrayrulewidth}
            &\multirow{2}{*}{Methods} & Sceneflow & KITTI 2012 & KITTI 2015 & Runtime \\
            & & EPE & 3px Out-All (\%) & D1-All (\%) & ($ms$)\\
            \hline
            % \hline
            \multirow{7}{*}{ \rotatebox{90}{\textit{Accuracy}}}
            &GC-Net~\cite{kendall2017end} & 2.51 & 2.30 & 2.87 & 900 \\ 
            % \cline{2-6}
            &CRL~\cite{pang2017cascade} & 1.32 & -- & 2.67 & \underbar{470} \\ 
            &SegStereo~\cite{yang2018segstereo} & 1.45 & 2.03 & 2.25 & 600 \\ 
            %&EdgeStereo~\cite{kendall2017end} & 2.51 & 2.30 & 2.16 & 700 \\ 
            % \cline{2-6}
            &PSMNet~\cite{chang2018pyramid} & 1.09 & \underbar{1.89} & 2.32 & \textbf{410} \\ 
            &PDS-Net~\cite{tulyakov2018practical} & 1.12 & 2.53 & 2.58 & 500 \\ 
            % \cline{2-6}
            &GANet-deep\cite{zhang2019ga} & \underbar{0.84} & \textbf{1.60} & \underbar{1.81} & 1,800 \\ 
            % \cline{2-6}
            &CSPN~\cite{cheng2018depth} & \textbf{0.78} & -- & \textbf{1.74} & 1,000 \\ 
            \hline
            % \hline
            \multirow{5}{*}{ \rotatebox{90}{\textit{Speed}}}
            &DispNetCorr~\cite{mayer2016large} & 1.68 & 4.65 & 4.34 & 60 \\ 
            % \cline{2-6}
            &DeepPrunerFast~\cite{duggal2019deeppruner} & 0.97 & -- & 2.59 & 62 \\
            % \cline{2-6}
            % &GANet-1~\cite{zhang2019ga} & 1.82 & 3.21 & -- & 67 \\ 
            % \cline{2-6}
            &StereoNet~\cite{khamis2018stereonet} & 1.101 & 6.02 & 4.83 & \textbf{15} \\ 
            % \cline{2-6}
            &AANet~\cite{xu2020aanet} & 0.87 & 2.42 & 2.55 & 62 \\ 
            % \cline{2-6}
            \rowcolor{red!7}
            &\textbf{LIGNet (Ours)} & \textbf{0.68} & \textbf{2.24} & \textbf{2.41} & \underbar{36} \\ 
            \Xhline{4\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Comparison with other state-of-the-arts models. \textbf{Bold}: Best, \underbar{Underbar}: Second best.}
    \label{table:comparison}
    \end{center}
\end{table*}

==> Tables/CostvolumeConstruction.tex <==
\begin{table}[t]
    \begin{center}
        \begin{adjustbox}{width=0.48\textwidth}
        \begin{tabular}{c|c|c|c}
            \Xhline{3\arrayrulewidth}
            \multicolumn{3}{c|}{SceneFlow EPE} &  \\ 
            \Xhline{3\arrayrulewidth}
            Construction method & No GCE & With GCE & Time $ms$ \\
            \Xhline{2\arrayrulewidth}
            % \hline
            Correlation & 1.020 & 0.863 & 26  \\
            Concatenation & 1.005 & 0.896 & 47 \\
            Gwc12 & 1.000 & 0.884 & 30 \\
            % \rowcolor{CuGray}
            \Xhline{3\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
    \caption{Effect of GCE on models with varying cost volume constructions methods.}
    \vspace{-7mm}
    \label{table:constructions}
    \end{center}
\end{table}

==> Tables/architecture.tex <==
\begin{table*}[h]
%\scriptsize
    \begin{center}
    %\vspace{-1cm}
        \begin{adjustbox}{width=0.99\textwidth}
        \renewcommand{\arraystretch}{1.}
        % \setlength{\tabcolsep}{6pt}
        \begin{tabular}{cl@{\hspace{2cm}}l@{\hspace{2cm}}l}
            \Xhline{3\arrayrulewidth}
            \textbf{No.} & \textbf{Layer Setting} & \textbf{Input} & \textbf{Output Dimension} \\
            \hline
            \hline
            \multicolumn{4}{c}{\textbf{Feature Extraction}} \\
            \Xhline{2\arrayrulewidth}
            $I$ & normalized image pair & & $H\times W\times 3$ \\ \noalign{\smallskip}
            (1-1) & \multirow{6}{*}{\bsplitcell{\\ \\ MobileNetV2 backbone \\ \\ \\ }}  & $I$ & $H/2\times W/2\times 16$ \\ \noalign{\smallskip}
            (1-2) &   & (1-1) & $H/4\times W/4\times 24$ \\ \noalign{\smallskip}
            (1-3) &   & (1-2) & $H/8\times W/8\times 32$ \\ \noalign{\smallskip}
            (1-4) &   & (1-3) & $H/16\times W/16\times 96$ \\ \noalign{\smallskip}
            (1-5) &   & (1-4) & $H/32\times W/32\times 160$ \\ \noalign{\smallskip}
            (2-4) & 2D deconv $4\times 4, 96$, stride 2, padding 1 & (1-5) & $H/16\times W/16\times 96$ \\ \noalign{\smallskip}
            $I^{(16)}$ & 2D conv $3\times 3, 192$ & concat (2-4) and (1-4) & $H/16\times W/16\times 192$ \\ \noalign{\smallskip}
            (2-3) & 2D deconv $4\times 4, 32$, stride 2, padding 1 & $I^{(16)}$ & $H/8\times W/8\times 32$ \\ \noalign{\smallskip}
            $I^{(8)}$ & 2D conv $3\times 3, 64$ & concat (2-3) and (1-3) & $H/8\times W/8\times 192$ \\ \noalign{\smallskip}
            (2-2) & 2D deconv $4\times 4, 24$, stride 2, padding 1 & $I^{(8)}$ & $H/4\times W/4\times 24$ \\ \noalign{\smallskip}
            $I^{(4)}$ & 2D conv $3\times 3, 48$ & concat (2-2) and (1-2) & $H/4\times W/4\times 48$ \\ \noalign{\smallskip}
            \hline
            \Xhline{2\arrayrulewidth}
            \multicolumn{4}{c}{\textbf{Cost Aggregation}} \\
            \Xhline{2\arrayrulewidth}
            $[1]$ & correlation layer & $I^{(4)}$ (Left and Right) & $48\times H/4\times W/4\times 1$ \\
            \Xhline{1\arrayrulewidth}
            $[2$-$1]$ & 3D conv $3\times 3\times 3, 8$ & $[1]$ & $48\times H/4\times W/4\times 8 $ \\
            $[2]$ & GCE & $[2$-$1]$ and $I^{(4)}$ & $48\times H/4\times W/4\times 8 $ \\
            $[3$-$1]$ & \bsplitcell{3D conv $3\times 3\times 3, 32$, stride 2 \\ 3D conv $3\times 3\times 3, 32$} & $[2]$ & $24\times H/8\times W/8\times 32 $ \\
            $[3]$ & GCE & $[3$-$1]$ and $I^{(8)}$ & $24\times H/8\times W/8\times 32 $ \\
            $[4$-$1]$ & \bsplitcell{3D conv $3\times 3\times 3, 64$, stride 2 \\ $2\times$ 3D conv $3\times 3\times 3, 64$} & $[3]$ & $12\times H/16\times W/16\times 64 $ \\
            $[4]$ & GCE & $[4$-$1]$ and $I^{(16)}$ & $12\times H/16\times W/16\times 64 $ \\
            $[5$-$1]$ & \bsplitcell{3D conv $3\times 3\times 3, 80$, stride 2 \\ 3D conv $3\times 3\times 3, 80$} & $[4]$ & $6\times H/32\times W/32\times 80 $ \\
            $[5]$ & GCE & $[5$-$1]$ and $I^{(32)}$ & $6\times H/32\times W/32\times 80 $ \\
            
            $[6$-$1]$ & 3D deconv $4\times 4\times 4, 64$, stride 2, padding 1 & $[5]$ & $12\times H/16\times W/16\times 64 $ \\
            $[6$-$2]$ & GSA & $[6$-$1]$ and $[4]$ and $I^{(16)}$ & $12\times H/16\times W/16\times 64 $ \\
            $[6$-$3]$ & 3D conv $3\times 3\times 3, 64$ & $[6$-$2]$ & $12\times H/16\times W/16\times 64 $ \\
            $[6]$ & GCE & $[6$-$3]$ and $I^{(16)}$ & $12\times H/16\times W/16\times 64 $ \\
            $[7$-$1]$ & 3D deconv $4\times 4\times 4, 32$, stride 2, padding 1 & $[6]$ & $24\times H/8\times W/8\times 32 $ \\
            $[7$-$2]$ & GSA & $[7$-$1]$ and $[3]$ and $I^{(8)}$ & $24\times H/8\times W/8\times 32 $ \\
            $[7$-$3]$ & 3D conv $3\times 3\times 3, 32$ & $[7$-$2]$ & $24\times H/8\times W/8\times 32 $ \\
            $[7]$ & GCE & $[7$-$3]$ and $I^{(8)}$ & $24\times H/8\times W/8\times 32 $ \\
            $[8]$ & 3D deconv $4\times 4\times 4, 1$, stride 2, padding 1 & $[7]$ & $48\times H/4\times W/4\times 1$ \\
            \hline
            \Xhline{2\arrayrulewidth}
            \multicolumn{4}{c}{\textbf{Regression}} \\
            \Xhline{2\arrayrulewidth}
            $\{1\}$ & Top-2 regression & $[8]$ & $48\times H/4\times W/4$ \\
            $\{2$-$1\}$ & \bsplitcell{2D deconv $4\times 4, 16$, stride 2, padding 1 \\ 2D deconv $4\times 4, 9$, stride 2, padding 1} & $I^{(4)}$ & $H\times W\times 9$ \\
            $\{2\}$ & `superpixel` upsampling & $\{2$-$1\}$ and $\{1\}$ & $H\times W$ \\
            \Xhline{2\arrayrulewidth}
        \end{tabular}
        \end{adjustbox}
        %\vspace{0.1cm}
    \caption{Network architecture.}
    \label{architecture}
    %\vspace{-1cm}
    \end{center}
\end{table*}
